Variational Transdimensional Inference

The expressiveness of flow-based models combined with stochastic variational inference (SVI) has expanded the application of optimization-based Bayesian inference to highly complex problems. However, despite the importance of multi-model Bayesian inference for problems defined on a transdimensional joint model and parameter space, such as Bayesian structure learning and model selection, flow-based SVI has been limited to problems defined on a fixed-dimensional parameter space. We introduce CoSMIC, normalizing flows (COntextually-Specified Masking for Identity-mapped Components), an extension to neural autoregressive conditional normalizing flow architectures that enables use of a single flow-based variational density for inference over a transdimensional (multi-model) conditional target distribution. We propose a combined stochastic variational transdimensional inference (VTI) approach to training CoSMIC, flows using ideas from Bayesian optimization and Monte Carlo gradient estimation. Numerical experiments show the performance of VTI on challenging problems that scale to high-cardinality model spaces.

==> sections/cosmic_composition_horizontal.tex <==
% ─── left-to-right version of your flow diagram ──────────────────────────────
\begin{tikzpicture}[
        >=latex, %>=stealth,
        node distance=\SF{0.45},  %\SF{0.65}% horizontal spacing
        baseline=0mm,
        auto,
        thin
]
\fiveTextFourMath
%──────────────────── nodes ────────────────────
\node[mRectStyle]                                (z)     {$\refvars$};
\node[mRectStyle,      above=\SF{0.8} of z]               (m)     {$\mdl$};

\node[mCircStyle, minimum height=\SF{0.95},      right=of z]                (Pm)    {$P_\mdl$};
\node[mHardRectStyle, right=of Pm]               (T1)    {$\transform_{\vipp}^{(1)}$};
\node[mNoBorder,       right=of T1]              (T2)    {$\uncdots$};
\node[mHardRectStyle,  right=of T2]              (T3)    {$\transform_{\vipp}^{(L)}$};
\node[mCircStyle, minimum height=\SF{0.95},      right=of T3]              (PmT)    {$P_\mdl^\top$};
\node[mRectStyle,      right=of PmT]             (theta)  {$\cvars,\auxvars_{\setminus\mdl}$};


% annotation nodes (optional)
\node[mNoBorder, above=of T1, yshift=\SF{1.2}]                    (cosmic1) {\method{} IAF step};
\node[mNoBorder, above=of T3, yshift=\SF{1.2}]                    (cosmic3) {\method{} IAF step};


\node[mNoBorder, below=of Pm, yshift=-\SF{1.2}]                    (perm) {Left-align permutation};
\node[mNoBorder, below=of PmT, yshift=-\SF{1.2}]                    (invperm) {Inverse left-align permutation};

%────────────────── arrows ─────────────────────
\foreach \src/\dst in {z/Pm, Pm/T1, T1/T2, T2/T3, T3/PmT, PmT/theta, m/T1}
  \draw[mArrowStyle] (\src) -- (\dst);

% extra influence from m to T3
\draw[mArrowStyle, bend left=15] (m) to (T3);

% dotted explanation lines
\foreach \src/\dst in {cosmic1/T1, cosmic3/T3, Pm/perm, PmT/invperm}
  \draw[dotted] (\src) -- (\dst);

%──────────────────── brace ────────────────────
\draw[
    decorate,
    decoration={brace,amplitude=6pt,raise=4pt},
] (PmT.south east) -- node[below=10pt] {$\transform_\vipp(\refvars\mid\mdl)$} (Pm.south west);


  % label in the top-left corner
  \node[anchor=north west,            % pin the anchor
        inner sep=0pt, outer sep=0pt, % no extra padding → box stays unchanged
        xshift=-2pt, yshift=11pt]      % (optional) small inset
        at (current bounding box.north west)
        {\scriptsize (a)};
\end{tikzpicture}

==> sections/cosmic_iaf_scaled.tex <==
%{\scalefont{0.1}%
\begin{tikzpicture}[
    >=latex, %>=stealth,
    %smallmath,
    node distance=\SF{0.5},
    baseline=0mm,
    auto,
    thin,
    %font=\fontsize{\SFp{10}}{\SFp{10.5}}\selectfont,
    edge/.style={->, thin},
    %smallfig,
]
\fiveTextFourMath

% --- Autoregressive NN block ---
\node[
      draw, 
      rectangle, 
      fill=green!20, 
      rounded corners,
      minimum width=\SF{2.3}, 
      minimum height=\SF{0.5}] (ann)
      {Autoregressive NN};

% --- m input ---
\node[draw, rectangle, fill=green!20, rounded corners,
      minimum width=\SF{0.5}, minimum height=\SF{0.5},
      left=\SF{1.0} of ann]                     (m) {$m$};

% --- rho nodes ---
\node[draw, rectangle, fill=green!20, rounded corners,
      below=\SF{0.5} of ann,
      minimum width=\SF{0.5}, minimum height=\SF{0.5}] (rho_ann) {$\rho$};

\node[draw, rectangle, fill=green!20, rounded corners,
      below left=\SF{0.5} and -\SF{0.8} of ann,
      minimum width=\SF{0.5}, minimum height=\SF{0.5}] (rhoId) {$\rho^{\mathrm{Id}}$};

% --- × nodes for convex combination ---
\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      below=\SF{0.5} of rho_ann]               (timesC) {$\boldsymbol{\times}$};

\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      below=\SF{1.6} of rhoId]                 (times1mC) {$\boldsymbol{\times}$};

% --- C(m) & 1‑C(m) nodes ---
\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      at={(m |- timesC)}]                     (ctm) {$C$};

\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      at={(m |- times1mC)}]                   (oneminusctm) {$-$};

\node[draw, rectangle, fill=green!20, rounded corners,
      minimum width=\SF{0.5}, minimum height=\SF{0.5},
      left=\SF{0.5} of oneminusctm]            (onevec) {$\boldsymbol{1}$};

% --- + node to combine ---
\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      right=\SF{1.5} of times1mC]              (combine) {$\boldsymbol{+}$};

% --- τ node ---
\node[draw, circle, inner sep=\SF{0.05},
      minimum width=\SF{0.45}, minimum height=\SF{0.45},
      below=\SF{0.5} of combine]               (tau) {$\tau$};

% --- z in/out ---
\node[draw, rectangle, fill=green!20, rounded corners,
      minimum width=\SF{0.5}, minimum height=\SF{0.5},
      at={(m |- tau)}]                        (z_in) {$\boldsymbol{z}$};

\node[draw, rectangle, fill=green!20, rounded corners,
      minimum width=\SF{0.5}, minimum height=\SF{0.5},
      right=\SF{1.0} of tau]                   (z_out) {$\boldsymbol{z}'$};

% --- edges (knot library keeps crossings tidy) ---
\begin{knot}[
%clip width=\SF{4}, 
clip width=2, 
consider self intersections,
ignore endpoint intersections=false,
end tolerance=\SF{1}, % keep proportional if desired
%every strand/.style={->, shorten >= -0.1cm}
]
  \strand[->, shorten >= -0.05cm] (ann) -- (rho_ann);
  \strand[->, shorten >= -0.05cm] (m)   -- (ann);
  \strand[->, shorten >= -0.05cm] (m)   -- (ctm);
  \strand[->, shorten >= -0.05cm] (ctm) -- (oneminusctm);
  \strand[->, shorten >= -0.05cm] (onevec) -- (oneminusctm);
  \strand[->, shorten >= -0.05cm] (ctm) -- (timesC);
  \strand[->, shorten >= -0.05cm] (oneminusctm) -- (times1mC);
  \strand[->, shorten >= -0.05cm] (z_in) -- (tau);
  \strand[->, shorten >= -0.05cm] (rho_ann) -- (timesC);
  \strand[->, shorten >= -0.05cm] (rhoId) -- (times1mC);
  \strand[->, shorten >= -0.05cm] (timesC) -| (combine);
  \strand[->, shorten >= -0.05cm] (times1mC) -- (combine);
  \strand[->, shorten >= -0.05cm] (combine) -- (tau);
  \strand[->, shorten >= -0.05cm] (tau) -- (z_out);
  \strand[->, shorten >= -0.05cm] (z_in)
      -- ++(0,\SF{0.4}) -- ++(\SF{0.65},0) -- ++(0,\SF{3.5}) -- (ann);
\end{knot}

% --- outer grey box ---
\node[draw=gray, thick,
      fit=(ann)(rho_ann)(rhoId)(tau),
      label=above:CoSMIC IAF\ step,
      inner sep=\SF{0.3}]                     (box) {};

% --- dotted sub‑box (ρ^C) ---
\node[draw, dotted,
      fit=(rho_ann)(rhoId)(onevec)(combine),
      label={[align=center, anchor=north east,
              inner sep=\SF{0.1}, xshift=\SF{0.02}, yshift=-\SF{0.02}]north east:
              $\rho^C$\\(eqn.~\ref{eqn:cosmic-rho-m})},
      inner sep=\SF{0.1}]                    {};

% --- adjust bounding box ---
\useasboundingbox
  (current bounding box.north west)
  rectangle
  ($(current bounding box.south east)+(0,\SF{2})$);

% label in the top-left corner
  \node[anchor=north west,            % pin the anchor
        inner sep=0pt, outer sep=0pt, % no extra padding → box stays unchanged
        xshift=-2pt, yshift=0pt]      % (optional) small inset
        at (current bounding box.north west)
        {\scriptsize (c)};
\end{tikzpicture}%
%}

==> sections/ctm_with_permutation_diagram.tex <==
\begin{tikzpicture}[
    >=latex, %>=stealth,
    node distance=\SF{0.45},
    baseline=0mm,
    auto,
    thin,
    edge/.style={->, thin},
]
\fiveTextFourMath
  %------------------------ nodes -------------------------------
  \node[mRectStyle] (m)  {$\mdl$};
  \node[minimum height=\SF{0.5},%\SF{0.9}, 
        right=\SF{0.7} of m,
        %label={[anchor=west]above:Example~input}
        ] 
        (mex) {\,\,\,\,\,\,\,\,\,\,\,5};
  %\node[above=of mex] (example) {\,\,Example input};
  \node[mCircStyle,  below=of m]   (A)  {$\modeltomask$};
  \node[mTensorStyle,right=\SF{0.7} of A]   (v1) 
    {$\left[\!\!\begin{array}{c}
    0\\[-1pt]
    0\\[-1pt]
    1\\[-1pt]
    0\\[-1pt]
    1\\[-1pt]
    \end{array}\!\!\right]$};
  \node[mCircStyle,  below=of A]  (Pm) {$P_\mdl$};
  \node[mTensorStyle,right=\SF{0.7} of Pm]  (v2) 
    {$\left[\!\!\begin{array}{c}
    1\\[-1pt]
    1\\[-1pt]
    0\\[-1pt]
    0\\[-1pt]
    0\\[-1pt]
    \end{array}\!\!\right]$};
  \node[mCircStyle,  below=of Pm]  (B)  {$\masktoapmask$};
  % \node[mTensorStyle,below=of B]   (M)  {$\left[\!\!\begin{array}{cccc}
  %    1&\cdots&1\\[-1pt]
  %    1&\cdots&1\\[-1pt]
  %    0&\cdots&0\\[-1pt]
  %    0&\cdots&0\\[-1pt]
  %    0&\cdots&0\\[-1pt]
  % \end{array}\!\!\right]$};
  \node[mTensorStyle,right=\SF{0.7} of B]   (M)  {$\left[\!\!\begin{array}{c}
     1\uncdots 1\\[-1pt]
     1\uncdots 1\\[-1pt]
     0\uncdots 0\\[-1pt]
     0\uncdots0\\[-1pt]
     0\uncdots 0\\[-1pt]
  \end{array}\!\!\right]^\top$};
  \node[mRectStyle, below=of B]    (xi) {$\ctm(\mdl)$};

  %------------------------ arrows ------------------------------
  %\foreach \src/\dst in {m/A, A/v1, A/Pm, Pm/v2, Pm/B, B/M, B/xi}
  %  \draw (\src) -- (\dst);
    %\draw[mArrowStyle] (\src) -- (\dst);
  
  \foreach \src/\dst in {m/A, A/Pm, Pm/B, B/xi}
    \draw[mArrowStyle] (\src) -- (\dst);
  
  \foreach \src/\dst in { A/v1,  Pm/v2,  B/M, m/mex}
    \draw[dotted] (\src) -- (\dst);

  %------------------------ big brace ---------------------------
  % \draw[diagram brace]%, xshift=5.2cm]
  %       (A.north west) -- node[mBraceTxtShift] {$\ctm$} (B.south west);
  % --- the brace --------------------------------------------------
  \draw[
          decorate,
          decoration={brace,amplitude=4pt,raise=4pt}, % raise = distance
          xshift=-3pt                                        % extra left offset
    ] (B.south west) -- node[left=10pt] {$\ctm$} (A.north west);

    %\draw[
     %     decorate,
     %     decoration={brace,amplitude=6pt,raise=4pt}, % raise = distance
     %     xshift=3pt                                        % extra left offset
    %] (mex.north east) -- node[right=10pt, rotate=-90, transform shape, anchor=mid] {Example input} (M.south east);
\draw[
  decorate,
  decoration={brace,amplitude=4pt,raise=0pt}, % mirror => brace on the right side for a top→bottom path
  xshift=0pt
] 
  ($(M.east |- mex.north)$) -- % x from M.east, y from mex.north  → top point
  node[right=8pt, rotate=-90, anchor=mid] {Example input}
  ($(M.east |- M.south)$);    % x from M.east, y from M.south     → bottom point (same as M.south east)

% label in the top-left corner
  \node[anchor=north west,            % pin the anchor
        inner sep=0pt, outer sep=0pt, % no extra padding → box stays unchanged
        xshift=-2pt, yshift=7pt]      % (optional) small inset
        at (current bounding box.north west)
        {\scriptsize (b)};
\end{tikzpicture}

